FruitProM-V2: Robust Probabilistic Maturity Estimation and Detection of Fruits and Vegetables

Accurate fruit maturity identification is essential for determining harvest timing, as incorrect assessment directly affects yield and post-harvest quality. Although ripening is a continuous biological process, vision-based maturity estimation is typically formulated as a multi-class classification task, which imposes sharp boundaries between visually similar stages. To examine this limitation, we perform an annotation reliability study with two independent annotators on a held-out tomato dataset and observe disagreement concentrated near adjacent maturity stages. Motivated by this observation, we model maturity as a latent continuous variable and predict it probabilistically using a distributional detection head, converting the distribution into class probabilities through the cumulative distribution function (CDF). The proposed formulation maintains comparable performance to a standard detector under clean labels while better representing uncertainty. Furthermore, when controlled label noise is introduced during training, the probabilistic model demonstrates improved robustness relative to the baseline, indicating that explicitly modeling maturity uncertainty leads to more reliable visual maturity estimation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/annotation_experiment.tex <==
\textbf{Annotation Experiment}
To evaluate model performance in tomato maturity estimation, a dataset of 400 images was curated, capturing tomatoes across three distinct maturity stages: ripe, half-ripe, and immature. To ensure variability and robustness in the dataset, images were collected under three different lighting conditions — daylight, night light, and sodium light — reflecting real-world scenarios in which such systems may be deployed. Each image contained multiple tomatoes at potentially varying stages of maturity, providing a challenging and representative set of samples for both annotation and subsequent model training and evaluation.

Four human subjects were recruited to independently annotate the entire dataset of 400 images without any collaboration or cross-referencing between annotators, ensuring that each annotation set remained unbiased by the judgments of others. The annotation procedure required each subject to draw a bounding box around every visible tomato in a given image and assign one of three class labels — ripe, half, or immature — based on their individual visual assessment. This multi-annotator design was intentionally adopted to capture inter-annotator variability, which is a known challenge in subjective labeling tasks such as maturity estimation, where the visual distinction between adjacent maturity stages can be ambiguous. The resulting annotations across all four subjects were subsequently used to assess annotator agreement and to establish a consensus ground truth for model benchmarking.





==> sec/discussion.tex <==



the noise induced by us acted as additional augmentation and helped smoothing out our probability distribution. 

==> sec/methodology/1_annoation_experiment.tex <==
\subsection{Annotation Reliability Study}

To evaluate the reliability of maturity annotations, we conducted an
inter-annotator agreement study on the tomato maturity test set.
Two independent annotators were asked to label each visible fruit
using the same three maturity categories employed in the original
dataset (unripe, intermediate, and ripe). The annotators performed
the labeling independently and were blinded to both the original
dataset annotations and each other’s decisions.

\subsubsection{Matching Procedure}

Because object detection produces sets of bounding boxes rather than
one-to-one correspondences, direct comparison of labels requires
associating detections across annotation sets. We therefore matched
annotated fruits using a bipartite assignment procedure based on
bounding box overlap.

Given two sets of annotations $A=\{a_i\}$ and $B=\{b_j\}$, we computed
the pairwise intersubsection-over-union (IoU) between all bounding boxes
and solved a minimum-cost matching problem using the Hungarian
algorithm \cite{Kuhn1955-pp,Frank2005-fw}. The optimal
assignment produces a one-to-one correspondence between fruits in the
two annotation sets. Only matched pairs with IoU above a threshold of
$\tau = 0.5$ were retained for analysis; unmatched detections were treated as
background and excluded from the reliability evaluation.

\subsubsection{Agreement Analysis}

Using the matched pairs, we constructed confusion matrices for:
\begin{itemize}
    \item Annotator A vs Annotator B,
    \item Annotator A vs original dataset labels,
    \item Annotator B vs original dataset labels.
\end{itemize}

This analysis isolates disagreement in maturity labeling while removing
localization differences between annotators.

\subsubsection{Purpose of Annotation Reliability Study}

The goal of this experiment is not to evaluate annotator performance,
but to evaluate the annotation process itself. If maturity were a
well-defined categorical state, independent annotators would produce
nearly identical labels after matching. Instead, disagreement indicates
that the observed label is a subjective measurement of an underlying
biological process.

In particular, we analyze where disagreement occurs across maturity
stages. Consistent disagreement concentrated between adjacent classes
suggests that maturity boundaries are gradual rather than discrete.
This observation motivates modeling maturity as a latent continuous
variable and treating the discrete label as an interval observation,
which directly informs the probabilistic formulation introduced in
Sec.~\ref{sec:problem_formulation}.

==> sec/related_works.tex <==

 \section{Related Work}

Deep learning has fundamentally reshaped fruit and vegetable maturity assessment, evolving from early CNN classification pipelines \cite{Garillos2021, Behera2021, Zhang2018Banana, Gao2020Strawberry} to high-speed YOLO and Transformer-based detectors \cite{Liu2020YOLOTomato, Zhao2025YOLODGS, Yang2023, Wu2025RTDETR}. While these models achieve high precision, they almost exclusively treat ripeness as a discrete classification task---a formulation fundamentally mismatched with the continuous, gradual nature of biological ripening. To address this, recent research into uncertainty quantification---using Bayesian approximation \cite{Gal2016}, deep ensembles \cite{Lakshminarayanan2017}, and evidential learning \cite{Sensoy2018Evidential, Amini2020DeepEvidential}---has begun to separate model ignorance (epistemic uncertainty) from inherent data noise (aleatoric uncertainty) \cite{Kendall2017Uncertainties}. Specialized probabilistic heads, such as Mixture Density Networks \cite{Bishop1994} and Beta-distribution regression \cite{Sadowski2019BetaDirichlet}, offer a mathematically grounded way to predict bounded, continuous attributes by providing a distribution over the maturity spectrum rather than a single point estimate.

The necessity of this probabilistic shift is further underscored by the inherent subjectivity of human annotation, where label noise around class boundaries can meaningfully degrade performance \cite{Frenay2014LabelNoise}. Agricultural literature confirms that inter-annotator disagreement is structural \cite{SadeghiTehran2017Wheat}, as phenological scales like BBCH describe processes that resist clean mapping onto discrete categories \cite{Meier2009BBCH, Bridgemohan2016BBCH}. Reducing multi-annotator responses to a single majority label discards vital signal; instead, learning over full response distributions or using soft probability targets \cite{Hinton2015Distilling, Peterson2019HumanUncertainty} produces better-calibrated models that generalize more reliably. By moving away from rigid one-hot labels toward continuous probabilistic supervision---leveraging techniques like label smoothing \cite{Szegedy2016LabelSmoothing} and ordinal-aware noise correction \cite{Garg2023OrdinalNoise}---models can finally account for the biological continuum and irreducible annotation noise, leading to more robust decision-making for harvest timing. 




==> sec/results.tex <==
Model Results 




Noise Study Rsults

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}
